Non-autoregressive Sequence-to-Sequence Vision-Language Models

Sequence-to-sequence vision-language models are showing promise, but their applicability is limited by their inference latency due to their autoregressive way of generating predictions. We propose a parallel decoding sequence-to-sequence vision-language model, trained with a Query-CTC loss, that marginalizes over multiple inference paths in the decoder. This allows us to model the joint distribution of tokens, rather than restricting to conditional distribution as in an autoregressive model. The resulting model, NARVL, achieves performance on-par with its state-of-the-art autoregressive counterpart, but is faster at inference time, reducing from the linear complexity associated with the sequential generation of tokens to a paradigm of constant time joint inference.

==> internal_comments.tex <==

(1) need to strongly justify the single token limitation of autoregressive models. Where is it shown that this standard practice is a limiting factor? If the sequence to be generated is not too complex we expect that the heavy lifting is done by the encoder.
     
Qi: Highlight the weakness of AR, like high latency as shown in exps, and also exposure bias,the error propagation (not agreed by Zhuowen)
   
(2) Arguing that this is more flexible but not showing improvements could be easy ground for the reviewer. 
        
        
(3) And an autoregressive model has by design higher capacity than a static model. Need to point to some references or show that choosing the fixed learnable prompts as X times larger than the AR embedding guarantees the static model has higher capacity. 
        
Qi: X times is not realistic to set, due to memory issue. but we can add exp for using same number of tokens as queries, but the tokens are from encoder.
        
        
(4) Introducing LQTs is in fact using prompt-tuning to change the behaviour of the decoder some comparison with prompt-tuning methods should be provided. 

Qi: add a paragraph to explain queries, and tell the difference between these queries and prompt-tuning.

(5) Moreover the distillation process (that appears to be key) suggest that NARVL can learn to closely mimic AR models, this makes the whole paper closer to distillation methods/model compression and the main thesis “we propose a novel architecture” gets weaker.

(6) Justify the fixed length output of the decoder, this is a limiting scenario (give some examples)
Qi: Do we explain how to choose this hyper-parameter in exp?

(7) The model is fine-tuned, not trained from scratch, this is more of an adaptation method than a new architecture that is pre-trained. 


(8)The larger the output sequence the worse the results, this could be interpreted as a huge limitation by the reviewers. Is it overfitting since the larger the output the higher the capacity? Or is it a limitation of the newly introduced loss/parametrization?

Qi: nice thougths, do we observe overfit on training? In my experiments, i did see the good performance on training, but not overfitting. 


(9) Since exposure bias is used a one of the motivations it should be addressed either with some experiments or in any case further described.
Qi: Can we find some visual example to illustrate the exposure bias issue in refcoco dataset? refcoco is the task we can outperform AR model.

[VIS]: refcoco: GT/AR/NAR box vis + tokens

(10) How to generate open ended captions/bboxes/...? If the model does not allow for open ended (in the length of the output sequence) or if the length is an hyper-parameter, this should be made clear as soon as possible. 

Qi: same as (6) 


(11) Line 349 typo
* Table 4/5/6 does not convey much if speed is not present for other models too. It is a clear sign that none of the methods from the literature has been tested on the evaluation benchmark (only OFA from which this paper is built). 
* Line 767, avoid using subjective adjectives “Amazing”
* Reference to Unified-IO is missing

------------
 Paper proposes a sequence to sequence vision-language model that leverages query tokens in the latent space. Authors show that proposed method can obtain on-par performance with autoregressive models with a significant boost up in inference latency. 
The problem is well motivated in the paper. It’s clear this paper addresses a problem of practical significance for VLMs. Adopting CTC loss for VLM decoding is a valid contribution. The paper demonstrates how the proposed method obtains on par performance with AR models at a lower latency on several tasks.
----------


(12) This paper can benefit from a proper ‘background’ section that introduces CTC loss and a description of how it is used in practice. At minimum, authors should consider referring readers to a proper source. 
Qi: Add CTC formulation in supp.

(13) Notation and explanation in section 3.2 is confusing and needs better clarification. Fig3 conveys a very little information. That space could’ve been used to illustrate how the CTC loss operates.

(14) It’ll be interesting to have a discussion on certain design choices made in the paper. For example, what’s the significance of using an architecture of form shown in Fig3 (c) as opposed to Fig3 (b)? Why is this design a better choice than BART style end to end decoder? 

Qi: this is related to (2)(3). Seems more discussions of pros and cons of the proposed decoder design. 

(15)It’ll be interesting to see how much of an impact distillation has on model performance - this should’ve been a part of the ablation.

 
(16) Figure 2 and Figure 3 should be swapped. The content in Figure 3 is first introduced in section 3.1, while some contents in Figure 2, such as the path and the q-ctc loss are introduced very lately. Therefore, seeing Figure 2 at current position is confusing.

(17) The description of Q-CTC loss is not very clear. For example, it does not describe how the valid path is created. Is there a rule to create valid paths by adding “-” and repeated characters? How many of them are required? Maybe an algorithm box will make it clear.

(18) In addition, what is a good intuition of the Q-CTC loss? What can be learned from the perturbed text? Some explanation and discussion is needed.

Qi: can we use visualization results to show the repeated tokens' benefits.
[VIS] output sequence.


